LLARVA: Vision-Action Instruction Tuning Enhances Robot Learning

In recent years, instruction-tuned Large Multimodal Models (LMMs) have been successful at several tasks, including image captioning and visual question answering; yet leveraging these models remains an open question for robotics. Prior LMMs for robotics applications have been extensively trained on language and action data, but their ability to generalize in different settings has often been less than desired. To address this, we introduce LLARVA, a model trained with a novel instruction tuning method that leverages structured prompts to unify a range of robotic learning tasks, scenarios, and environments. Additionally, we show that predicting intermediate 2-D representations, which we refer to as "visual traces", can help further align vision and action spaces for robot learning. We generate 8.5M image-visual trace pairs from the Open X-Embodiment dataset in order to pre-train our model, and we evaluate on 12 different tasks in the RLBench simulator as well as a physical Franka Emika Panda 7-DoF robot. Our experiments yield strong performance, demonstrating that LLARVA - using 2-D and language representations - performs well compared to several contemporary baselines, and can generalize across various robot environments and configurations.

==> sections/dataset.tex <==
\section{Dataset}
\label{sec:dataset}

==> sections/intro-backup.tex <==

\def\figPipeline#1{
    \captionsetup[sub]{font=small}
    \begin{figure*}[#1]
      \centering
      \includegraphics[width=\linewidth]{Figure/Pipeline.pdf}
      % \vspace{-6pt}
      \caption{Overview of \Ours. We format the robot manipulation task as a Question \& Answer problem. In our pre-training, we prompt the model via a language template which has the {\texttt{\color{robottype}``robot model''}}, {\texttt{\color{controltype}``control mode''}}, {\texttt{\color{robottask}``robot task''}},{\texttt{\color{robotaction}``robot action''}}, and 
      {\texttt{\color{predsteps} `` number of predicted steps''}} as variables, achieving scalable pre-training on a mixed data source. When evaluating the model on a specific downstream task, the modules marked as \raisebox{-0.5ex}{\includegraphics[height=2.7ex]{Figure/fire.png}} are tunable given few shots of downstream demonstrations.}
      % \vspace{-0.3cm}
      \label{fig:teaser}
    \end{figure*}
}


\section{Introduction}
\label{sec:intro}

% \yuvan{Large Language Models or Large Multimodal Models?}

%1. Recently, LMMs

%2. However, r

Recently, instruction-tuned Large Multimodal Models (LMMs), such as InstructBLIP~\cite{instructblip}, InstructGPT~\cite{InstructGPT_ouyang2022training}, LLaVA~\cite{liu2023llava, liu2023llava15}, PALM~\cite{Chowdhery2022PaLMSL} and others have demonstrated state-of-the-art performance on a variety of vision-and-language tasks. However, existing LMMs for robotics~\cite{Driess2023PaLMEAE,shridhar2023perceiver,team2024octo,Brohan2023RT2VM} do not always demonstrate the same success and consistency across various embodied settings. This may result from the unique challenges encountered in robotics, such as the variability of real-world environments, the differences between robots, and the need to control actions reliably. Since LMMs have been proven to be successful in part due to multimodal instruction tuning, it is natural to leverage this technique in a robotics setting as well. Here, we propose that Vision-Action Instruction Tuning can bridge the gap between a language model's fundamental pre-training objective—next-word prediction—and the goal of enabling the model to handle various robotics settings.



% In this work, we introduce LLaRVA, an instruction-tuned LMM for robotic applications that can be generalized across various environments. To achieve this, we must align two different modalities: the visual (i.e., pixels or voxels) and the physical world (i.e., action trajectory). We choose to align these modalities using visual-action instructions. \tjd{ These lines are unclear:} But, in order to construct such instructions, it is crucial to use accessible, non-costly data that is easily found across domains and can be readily expressed as instructions. Recent works have used 3D representations such as voxels~\cite{shridhar2023perceiver} and point clouds~\cite{guhur2023instruction}. However, collecting 3D annotations is costly and difficult across multiple robots and environments, especially when large amounts of data are involved. \tjd{...and the point needs to be made more clearly/sharply.  What exactly is the limitation of the previous methods?  Which are the previous methods?  You haven't cited anything...}



% LLaRVA: a Large Language model for Robotic Vision and Action
% the motivation of leveraging language instruction format for ...

In this work, we introduce {\smodel}, an open-source instruction-tuned LMM for robotic applications that can generalize efficiently across various environments. Our key idea is the formulation of a novel instruction prompt that encapsulates robot type, task, scene configuration, and control regime in a natural language prefix amenable to contemporary LMMs.  We present an instruction tuning procedure tailored to the robotic domain --- when given an instruction that describes the ``robot model'', ``control mode'', ``robot task'', and ``robot action'', the model needs to anticipate future actions and the resulting visual trace using a language format. This architecture allows us to leverage language as the ``lingua franca'' of robotic perception and control (See Figure XX).


% However, aligning the visual and action modalities to produce meaningful robotic outputs is still not a trivial task. Recent robotic instruction-based works have successfully used 3D representations such as voxels~\cite{shridhar2023perceiver} and point clouds~\cite{guhur2023instruction}, but these modalities can be expensive to obtain and/or are not easily incorporated into most existing LMMs. 

%3
However, aligning the vision and action modalities to produce meaningful robotic outputs is still not a trivial task. Recent robotic LMMs have successfully used 3D representations such as voxels~\cite{shridhar2023perceiver} and point clouds~\cite{guhur2023instruction}. However, the 3D representations are not only difficult to incorporate into most existing LMMs, but are also costly to obtain, making it prohibitively expensive to scale training.  Hence, here, we utilize 2D camera data, which is easy to scale and integrate with existing LMMs.


% Hence, it is crucial that we utilize accessible data that is not costly to annotate and can be found easily for vision-action instructions. 



% the flow here:
% 2 - our key idea is one language-based instruction that is great bla bla
% 3 - aligning the modalities -> recent robotic LMMs used 3D -> but the annotations costly -> so, we want to use that 
% 4 - 2D representations -> visual traces -> auxiliary task


% - 3d is expensive DONE
% - so we use 2d
% - in order to make to 2d work better, we align with the visual traces

%4
We find that predicting an intermediate 2D representation, which we refer to as visual traces, can help align the vision and action spaces across different robot and task configurations. In particular, we generate the 2D visual trace (projection) of an end effector and force the model to predict this trace alongside the next robot action. We conjecture that this waypoint prediction helps to learn an aligned vision and action representation, enabling the model to better focus on the most important area and resulting in a more accurate prediction of robot actions. We construct instructions with such visual traces using the Open-X Embodiment dataset (OXE)~\cite{open_x_embodiment_rt_x_2023}, carefully categorizing the action space, the robot type, and control type.


% We also find in our work that predicting the 2-D projection of actions in the scene can further improve generalization.  We conjecture this is a useful waypoint prediction task which additionally unifies the learned representation (See Figure 3.)



% To achieve this, we align  2D visual inputs and the physical world (i.e., action trajectories) using visual-action instructions (See Figure 1).
%But, in order to construct such instructions, it is crucial to use accessible, non-costly data that is easily found across domains and can be readily expressed as instructions. 

%collecting 3D annotations is costly and difficult across multiple robots and environments, especially when large amounts of data are involved. \tjd{...and the point needs to be made more clearly/sharply.  What exactly is the limitation of the previous methods?  Which are the previous methods?  You haven't cited anything...}



% % 3
% In this work, we introduce \smodel: a Large Language model for Robotic Vision and Action, an open-source instruction-tuned LMM for robotic applications that can generalize efficiently across various environments. To achieve this, we align  2D visual inputs and the physical world (i.e., action trajectories) using visual-action instructions (See Figure 1).
% %But, in order to construct such instructions, it is crucial to use accessible, non-costly data that is easily found across domains and can be readily expressed as instructions. 
% Recent robotic instruction-based works have successfully used 3D representations such as voxels~\cite{shridhar2023perceiver} and point clouds~\cite{guhur2023instruction}, but these modalities can be exensive to obtain and/or are not natively present in most existing vision-and-language LMMs. 
% %collecting 3D annotations is costly and difficult across multiple robots and environments, especially when large amounts of data are involved. \tjd{...and the point needs to be made more clearly/sharply.  What exactly is the limitation of the previous methods?  Which are the previous methods?  You haven't cited anything...}






% Our key idea is the formulation of a novel vision action instruction tunin prompt which encapsulates robot geometry, task, scene configuration, and control regime in a natural language prefix amenable to contemporary LMMs.  We present an instruction tuning procedure tailored to the robotic domain --- when given an instruction that describes the ``robot model'', ``control mode'', ``robot task'', and ``robot action'', the model needs to anticipate future actions and the resulting visual trace using a language format. This architecture allows us to leverage language as the 'lingua franca' of robotic perception and control (See Figure 2.)

% Therefore, we leverage a 2D end-effector visual trace, as image data is widely available, while 3D information is not.

% However, aligning these two modalities would usually require 3D annotations, such as voxels and depth, which could be highly expensive and difficult to collect. This becomes even more evident when collecting data on a large scale in robotic environments, which are notorious for having a limited amount of data compared to standard vision benchmarks. Hence, in order to construct visual-action instructions for robotics that align these two modalities, it is crucial that we utilize accessible data that is not costly to annotate and can be found easily in these domains.


% Thus, a key aspect of constructing visual-action instruction data for robotics that aligns these two modalities is to rely on that does not require expensive annotations.


% 2 - 2D visual trace + language as a bridge

% We also find in our work that predicting the 2-D projection of actions in the scene can further improve generalization.  We conjecture this is a useful waypoint prediction task which additionally unifies the learned representation (See Figure 3.)
%to service. %it is also possible to 
%align these two modalities effectively with instructions using fine-grained 2D localization. Specifically, the model predicts both the action and the 2D visual trace of a gripper using next-token prediction. With the help of a simple detector, \tjd{This is a red flag I would NOT put this in the introduction.  You could also have rendered the projection of the end effector.  Just saw we know or can estimate projection of the end effector in the image, and in the implementation section reveal the detector} we can generate pseudo-labels for the visual trace using a 2D projection of the gripper's 3D trajectory. Through this approach, we demonstrate that the model can focus on the most relevant areas, resulting in a more accurate prediction of robot action. Encouraged by this, we construct a new visual-action instruction dataset based on the Open X-Embodiment dataset (OXE) from a diverse collection of 37 OXE subsets with 13 different robots, carefully categorizing the robot type, robot mode, robot task, and robot action, as well as including the visual traces of the end effector.
% Encouraged by this, we construct a new visual-action instruction dataset based on the Open X-Embodiment dataset (OXE)~\cite{open_x_embodiment_rt_x_2023}, carefully categorizing the robot type, robot mode, robot task, and robot action while d, as well as the visual traces of the end effector from a diverse collection of 37 OXE subsets with 13 different robots. 
% This results in a new visual-action instruction dataset of 8M images and visual traces. 
% Here, we find that aligning these two modalities using fine-grained localization is an effective way to bridge the gap. 
% In particular, we generate the 2D visual trace (projection) of a gripper and constrain  the model to predict the trace using next-token prediction. As a result of the 2D visual trace prediction, we demonstrate that the model can better focus on the area that is most important, resulting in a more accurate prediction of robot actions. We construct instructions with such visual traces using  on the Open-X Embodiment dataset (OXE)~\cite{open_x_embodiment_rt_x_2023}, carefully categorizing the action space, the robot type, control type.
%Additionally, we trained a detector to get all the 2D visual traces of the end effector.

% Add this here: the prediction of the 2D visual trace enables the model to better focusing on the most important area and understand how to achieve the goal.

% Also this: We contribute a dataset, unified previous OXE by carefully categorizing the action space, the robot type, control type. We train a gripper detector to get all the 2D visual traces of the end effector.




% % 4 - recent research ?
% % OCTO,VLM-A, PERACT, GR-1
% Recent research...


% 4 - Our method
%Our method can be described as follows.
% See~\figref{fig:teaser} for an overview. We emphasize two key aspects of the instruction format used in our approach. First, we utilize the instruction language format as a universal interface for training a general-purpose agent to switch between different robot models, control modes, actions, and tasks in an end-to-end manner. Furthermore, we have found that instruction-tuned LMMs can be utilized more effectively by predicting future actions and visual traces expressed as natural language, similar to their counterpart vision-and-language LMMs.











% Key Contributions: 

% 1. language formatting enables merging different dataset especially across different robot type, different control type, different action space, bridge the domain gap and better use the current mixed dataset like OXE

% 2. 2D visual Trace joint training introduces visual instructural bias enabling the model better focusing on most important area and understand how to achieve the goal

% 3. We contribute a dataset, unified previous OXE by carefully categorizing the action space, the robot type, control type. We train a gripper detector to get all the 2D visual traces of the end effector.
% %===============================================================================



\figPipeline{t!}


% present instructed data model, 

%We summarize our main contributions as follows: 
%(i) We present the first instruction-tuned LMM for robot learning using instruction language format by aligning the visual-action multimodal spaces.
%(ii) We show that {\smodel} is easily applicable to robots across various environments, robot control types, and domains.
% Using our {\smodel}, we show robots that can be integrated into a variety of environments, control types, and domains.
%(iii) We present a new visual-action instruction dataset based on OXE, containing 8.5M image-2D visual trace pairs to facilitate future research. 
%(iv) {\smodel} demonstrates generalization across different simulated robots and environments, yielding improved performance.



==> sections/intro_old.tex <==

\def\figPipeline#1{
    \captionsetup[sub]{font=small}
    \begin{figure*}[#1]
      \centering
      \includegraphics[width=\linewidth]{Figure/Pipeline.pdf}
      % \vspace{-6pt}
      \caption{Overview of \Ours. We format the robot manipulation task as a Question \& Answer problem. In our pre-training, we prompt the model via a language template which has the {\texttt{\color{robottype}``robot model''}}, {\texttt{\color{controltype}``control mode''}}, {\texttt{\color{robottask}``robot task''}},{\texttt{\color{robotaction}``robot action''}}, and 
      {\texttt{\color{predsteps} `` number of predicted steps''}} as variables, achieving scalable pre-training on a mixed data source. When evaluating the model on a specific downstream task, the modules marked as \raisebox{-0.5ex}{\includegraphics[height=2.7ex]{Figure/fire.png}} are tunable given few shots of downstream demonstrations.}
      % \vspace{-0.3cm}
      \label{fig:teaser}
    \end{figure*}
}


\section{Introduction}
\label{sec:intro}

% \yuvan{Large Language Models or Large Multimodal Models?}

%1. Recently, LMMs

%2. However, r

Recently, instruction-tuned Large Multimodal Models (LMMs), such as LLaVA~\cite{liu2023llava, liu2023llava15}, InstructBLIP~\cite{instructblip}, and others have demonstrated state-of-the-art performance on a variety of vision-and-language (VL) tasks. However, existing LMMs for robotics~\cite{Driess2023PaLMEAE,shridhar2023perceiver,team2024octo,Brohan2023RT2VM} do not demonstrate this same success and consistency across various embodied settings. This may result from the unique challenges encountered in robotics, such as the variability of real-world environments, the differences between robots, and the need to control actions reliably. Since LMMs are successful in VL due to multimodal instruction tuning (IT), it is natural to leverage this technique in a robotics setting as well. IT can bridge the gap between the language model's fundamental pre-training objective—next-word prediction—and our goal of enabling the model to handle the variance of different robotics settings.

% IT can bridge the gap between the language model decoder's pre-training fundamental objective --- next-word prediction --- and our goal of enabling the model to handle the variance of different robotics settings.
% Since LMMs are successful in VL due to multimodal instruction tuning to align with human intents, it is natural to leverage instruction fine-tuning to align the reasoning structure of LMMs to handle the variance of different robotics settings.



% Since LMMs are successful in VL due to multimodal instruction tuning to align with human intents, it is natural to similarly align the reasoning structure of LMMs in robotics by leveraging instruction fine-tuning.


%This success is largely due to their ability to follow multimodal instructions aligned with human intent. 


% However, when it comes to existing LMMs for robotics, it is still unclear how to leverage instruction fine-tuning in order to generalize across a wide range of robotic learning tasks, scenarios, and environments without policy training. 

% A natural question arises as to whether developing an instruction-tuned LMM for the robotics domain is possible. And if so, how?

% Chancharik's suggestion
% However, when it comes to existing LMMs for robotics, the standard approach is to familiarize the model with the different modalities of embodied data via pretraining or prompting. 
% The underlying format of the reasoning of the model whether via natural language or code generation is still aligned for VL tasks. 
% Thus, to leverage LMMs for robotics, we propose utilizing instruction finetuning to actually structure the reasoning of LMMs for general embodied tasks.

% Recently, instruction-tuned Large Multimodal Models (LMMs), such as LLaVA~\cite{liu2023llava, liu2023llava15},  BLIP~\cite{instructblip,li2023blip2}, and others have demonstrated state-of-the-art performance on a variety of vision-and-language (VL) tasks. This is mainly due to their ability to follow multi-modal instructions that are aligned with human intents for performing a wide range of tasks. Despite these models showing tremendous success in VL tasks, they have not yet been demonstrated to work in the robotic domain. This may be a result of the challenges encountered in the robotic domain, such as the variability of real-world environments, the differences between robots, and the need to control actions reliably. A natural question arises as to whether developing an instruction-tuned LMM for the robotic domain is possible. If so, how?

% the robotics domain still has not reached the same level of proficiency. In particular, the robotic domain often faces unique challenges such as real-world variability, differences in robots and environments, and reliable control over physical actions. 

% % Aligning these modalities without instructions has been accomplished in other recent works~\cite{shridhar2023perceiver} using 3D representations, such as voxels, depth, and more. 

% While aligning these modalities has been accomplished in other recent works~\cite{shridhar2023perceiver} using 3D representations, such as voxels, depth, and more, we used a different approach using instructions.
% in robotic environments, which are notorious for limited data compared with standard vision benchmarks. 

% 1- aligning the multimodal visual and action spaces. visual-action instructions

% rewrite the paragraph

% In this work, we introduce LLaRVA, an instruction-tuned LMM for robotic applications that can be generalized across various environments. To achieve this, we must align two different modalities: the visual (i.e., pixels) and the physical world (i.e., action trajectory). Here, we aligned these modalities using instructions, while recent works~\cite{shridhar2023perceiver} have used 3D representations such as voxels, depth, and more. Nevertheless, 3D annotations are highly expensive and difficult to collect across multiple robots and environments, particularly when collecting large amounts of data. Even if one is able to collect the necessary data, it is not clear how to convey 3D information within visual instructions as it is not clear how 3D should be expressed. Hence, in order to construct visual-action instructions for robotics that align these two modalities, it is not only crucial that we use accessible and non-costly data that can be found easily across domains, but also that can be readily expressed in the form of instructions.

In this work, we introduce LLaRVA, an instruction-tuned LMM for robotic applications that can be generalized across various environments. To achieve this, we must align two different modalities: the visual (i.e., pixels or voxels) and the physical world (i.e., action trajectory). We choose to align these modalities using visual-action instructions. \tjd{ These lines are unclear:} But, in order to construct such instructions, it is crucial to use accessible, non-costly data that is easily found across domains and can be readily expressed as instructions. Recent works have used 3D representations such as voxels~\cite{shridhar2023perceiver} and point clouds~\cite{guhur2023instruction}. However, collecting 3D annotations is costly and difficult across multiple robots and environments, especially when large amounts of data are involved. \tjd{...and the point needs to be made more clearly/sharply.  What exactly is the limitation of the previous methods?  Which are the previous methods?  You haven't cited anything...}




% Therefore, we leverage a 2D end-effector visual trace, as image data is widely available, while 3D information is not.

% However, aligning these two modalities would usually require 3D annotations, such as voxels and depth, which could be highly expensive and difficult to collect. This becomes even more evident when collecting data on a large scale in robotic environments, which are notorious for having a limited amount of data compared to standard vision benchmarks. Hence, in order to construct visual-action instructions for robotics that align these two modalities, it is crucial that we utilize accessible data that is not costly to annotate and can be found easily in these domains.


% Thus, a key aspect of constructing visual-action instruction data for robotics that aligns these two modalities is to rely on that does not require expensive annotations.


% 2 - 2D visual trace + language as a bridge

We find in our work that it is also possible to align these two modalities effectively with instructions using fine-grained 2D localization. Specifically, the model predicts both the action and the 2D visual trace of a gripper using next-token prediction. With the help of a simple detector, \tjd{This is a red flag I would NOT put this in the introduction.  You could also have rendered the projection of the end effector.  Just saw we know or can estimate projection of the end effector in the image, and in the implementation section reveal the detector} we can generate pseudo-labels for the visual trace using a 2D projection of the gripper's 3D trajectory. Through this approach, we demonstrate that the model can focus on the most relevant areas, resulting in a more accurate prediction of robot action. Encouraged by this, we construct a new visual-action instruction dataset based on the Open X-Embodiment dataset (OXE) from a diverse collection of 37 OXE subsets with 13 different robots, carefully categorizing the robot type, robot mode, robot task, and robot action, as well as including the visual traces of the end effector.



% Encouraged by this, we construct a new visual-action instruction dataset based on the Open X-Embodiment dataset (OXE)~\cite{open_x_embodiment_rt_x_2023}, carefully categorizing the robot type, robot mode, robot task, and robot action while d, as well as the visual traces of the end effector from a diverse collection of 37 OXE subsets with 13 different robots. 



% This results in a new visual-action instruction dataset of 8M images and visual traces. 

% Here, we find that aligning these two modalities using fine-grained localization is an effective way to bridge the gap. In particular, we generate the 2D visual trace of a gripper self-supervised and force the model to predict using next-token prediction. As a result of the 2D visual trace prediction, we demonstrate that the model can better focus on the area that is most important, resulting in a more accurate prediction of robot actions. Encouraged by this, we construct a new visual-action instruction dataset that contains instructions based on the Open-X Embodiment dataset (OXE)~\cite{open_x_embodiment_rt_x_2023}, carefully categorizing the action space, the robot type, control type. Additionally, we trained a detector to get all the 2D visual traces of the end effector.

% Add this here: the prediction of the 2D visual trace enables the model to better focusing on the most important area and understand how to achieve the goal.

% Also this: We contribute a dataset, unified previous OXE by carefully categorizing the action space, the robot type, control type. We train a gripper detector to get all the 2D visual traces of the end effector.




% % 4 - recent research ?
% % OCTO,VLM-A, PERACT, GR-1
% Recent research...


% 4 - Our method
Our method can be described as follows. We present an instruction tuning procedure tailored to the robotic domain --- when given an instruction that describes the ``robot model'', ``control mode'', ``robot task'', and ``robot action'', the model needs to anticipate future actions and the resulting visual trace using a language format. See~\figref{fig:teaser} for an overview. We emphasize two key aspects of the instruction format used in our approach. First, we utilize the instruction language format as a universal interface for training a general-purpose agent to switch between different robot models, control modes, actions, and tasks in an end-to-end manner. Furthermore, we have found that instruction-tuned LMMs can be utilized more effectively by predicting future actions and visual traces expressed as natural language, similar to their counterpart vision-and-language LMMs.











% Key Contributions: 

% 1. language formatting enables merging different dataset especially across different robot type, different control type, different action space, bridge the domain gap and better use the current mixed dataset like OXE

% 2. 2D visual Trace joint training introduces visual instructural bias enabling the model better focusing on most important area and understand how to achieve the goal

% 3. We contribute a dataset, unified previous OXE by carefully categorizing the action space, the robot type, control type. We train a gripper detector to get all the 2D visual traces of the end effector.
% %===============================================================================



\figPipeline{t!}


% present instructed data model, 

We summarize our main contributions as follows: 
(i) We present the first instruction-tuned LMM for robot learning using instruction language format by aligning the visual-action multimodal spaces.
(ii) We show that {\smodel} is easily applicable to robots across various environments, robot control types, and domains.
% Using our {\smodel}, we show robots that can be integrated into a variety of environments, control types, and domains.
(iii) We present a new visual-action instruction dataset based on OXE, containing 8.5M image-2D visual trace pairs to facilitate future research. 
(iv) {\smodel} demonstrates generalization across different simulated robots and environments, yielding improved performance.


==> sections/mothod_v1_old.tex <==

\def\figPipeline#1{
    \captionsetup[sub]{font=small}
    \begin{figure*}[#1]
      \centering
      \includegraphics[width=\linewidth]{Figure/Pipeline.pdf}\vspace{-6pt}
      \caption{Overview of \Ours. We format the robot manipulation task as a Question \& Answer problem. In our pre-training, we prompt the model via a language template which has the {\texttt{\color{robottype}``robot model''}}, {\texttt{\color{controltype}``control mode''}}, {\texttt{\color{robottask}``robot task''}},{\texttt{\color{robotaction}``robot action''}}, and 
      {\texttt{\color{predsteps} `` number of predicted steps''}} as variables, achieving scalable pre-training on a mixed data source. When evaluating the model on a specific downstream task, the modules marked as \raisebox{-0.5ex}{\includegraphics[height=2.7ex]{Figure/fire.png}} are tunable given few shots of downstream demonstrations.
      }
      \label{fig:pipeline}
    \end{figure*}
}

\def\figDatainfo#1{
    \captionsetup[sub]{font=small}
    \begin{figure*}[#1]
      \centering
      \includegraphics[width=\linewidth]{Figure/datainfo.pdf}\vspace{-6pt}
      \caption{We contribute a large visual robotics dataset built upon Open-X Embodiment~\cite{padalkar2023open}, including 8.5M image-2D visual trace pairs. The left side shows some samples of the visual observations and 2D visual traces with the corresponding robot type and control mode. The right side shows the distribution of our dataset.
      }
      \label{fig:teaser}
    \end{figure*}
}











\section{Large Language Model for Robotic Vision and Action (LLaRVA)}
\label{sec:method}



% To address the challenge of performing many-shot multimodal in-context learning, we demonstrate the existence of {\smodel} in LMMs and then leverage them for many-shot multimodal ICL. 
% We begin by describing some background on multimodal ICL and task vectors (\Secref{sec:MTV:preliminaries}). We then introduce our three-step approach: (i) We calculate the mean activations of the attention heads from the many-shot multimodal ICL examples (\Secref{sec:MTV:mu}); (ii) We then extract the set of LMM attention heads locations that best align to the downstream task using an adapted version of the REINFORCE~\cite{Williams2004SimpleSG} algorithm (\Secref{sec:MTV:mtvextract}); and (iii) We replace the calculated mean activation values into the LMM for a downstream task (\Secref{sec:MTV:mtvapp}). The method overview is also illustrated~\figgref{fig:overview}.


\figPipeline{t!}

\subsection{Preliminaries}
\label{subsec:Preliminaries}


% the basic architecture of transformers, and inputs O_t and l

We formulate our language-conditioned visual robot manipulation as learning a robot agent $\mathcal{\pi}$, that takes the current visual observation image $o_t$ and the language instruction $l$  as input and predicts the action of the current step $a_{t}$ and the future 2D visual traces of the end effector (as defined in Section \ref{subsec:2dtraces}) from the current step to the end of the task  $tr_{t:g}$.

\begin{align}
\pi(o_t, l) \to a_t, tr_{t:g}
\label{eqn:model_formulation}
\end{align}

The language instruction $l$ includes two parts: the task description (\textit{e.g.} ``pick the bottle from the bottom drawer'') and robots states $s_{t-h:t}$ (\textit{i.e.} a list of previous joint positions or end effector positions and gripper states, where $h$ is the number of previous steps the model should be conditioned on). Different from all previous work, we formulate the proprioceptive information using language via a template shown in ~\cref{fig:pipeline}. This novel language-based approach frees the model architecture to profit from more diverse training samples in terms of different robots and their action spaces.  The model then has the potential to be scalable in terms of both data amount and model size, as opposed to the more conventional technique of using specifically trained action tokenizers, which require adhering to a rigid format. \dantong{move it to somewhere later}


\subsection{2D Visual Traces}
\label{subsec:2dtraces}
We define 2D visual traces to be a set of coordinates in 2D space aligned with the input visual observation:


\begin{equation}
tr_{t:g} = [(x_t, y_t), (x_{t+1}, y_{t+1}), ..., (x_{g}, y_{g})]
\label{eqn:2dtrace}
% \end{align}
\end{equation}

The model predicts the visual trace from current timestep $t$ to the last timestep $g$ when the goal of the instruction is achieved.  In order to predict such a trace of the end effector, the model needs to understand the task and plan the route to achieve that goal, both in terms of temporal space (number of future steps) and Cartesian space (the physical route taken). The 2D trace information thus helps the model align the visual space and the robot action space, leading to a more comprehensive understanding of the inputs to achieve better performance.
% \subsection{Large Scale Pre-training via Language}



\subsection{LLaRVA Agent}


\minisection{Architecture} We show the architecture of \Ours\ in~\cref{fig:pipeline}. The visual observation is processed through a frozen vision encoder to extract visual features, which are further projected into a hidden latent space matched with the dimensionality of the language tokens. The language instruction is tokenized using a word tokenizer. Then, the visual tokens and word tokens are concatenated and fed into Transformers, which are trained for next token prediction.

\minisection{Step 1: Large Scale Pre-training via Language} Thanks to language, we build a unified model architecture that can be trained on mixed data. As 
 mentioned in Section \ref{subsec:Preliminaries}, current large robotics models like Octo \cite{team2024octo} \yuvan{if we remove the extra part from 2.1, rewrite this part} that are trained on mixed data need to map the robot proprioceptive information and predicted actions to the same space. Since the model architecture is fixed, inputs and outputs must always follow their respective dimensions and semantic meanings. However, due to variability in factors like data collection processes and environments (\ie lighting, background, camera fps), formatting of post-processed data, robot types, and control mode (\ie joint control v.s. end effector control), mapping the data from different sources to the same space is impractical, and can even cause confusion while training. With \Ours, we create a template to transfer the actions in different latent spaces to a unified language space as shown in~\cref{fig:pipeline}. In the pre-training stage, we take the unified data samples as inputs and leverage autoregressive next token prediction to model the robotic manipulation task.


\minisection{Step 2: Fine-tuning for Downstream Tasks} The pre-trained model can be used for downstream tasks after fine-tuning on a small dataset with specific configurations for all the factors mentioned above. Having seen diverse data samples makes it easy for the model to adapt to specific downstream settings that resemble what it has already encountered in pre-training.


% We find that pre-training can help improve performance; this is further discussed in the ablations presented in Section \ref{sec:eval:ablations}.



\subsection{Visual-Action Instruction Dataset}

\figDatainfo{t!}


For our large language visual robotics pre-training, we contribute a customized dataset built from Open-X Embodiment~\cite{padalkar2023open}. As shown in~\cref{fig:datainfo}, our dataset consists of 8.5 million visual observations from a diverse collection of 37 OX-E subsets with 13 different robots. We include subsets that use two different control modes: end-effector control and joint control. For each visual observation, the 2D visual trace of the end-effector from the current step to the end of the task is also included.  


% This is calculated using the center points of bounding boxes found with an end-effector detector that we trained specifically for this OXE split.

==> sections/supp_v2.tex <==
\def\figDatainfo#1{
    \captionsetup[sub]{font=small}
    \begin{figure*}[#1]
      \centering
      \includegraphics[width=\linewidth]{Figure/chart.pdf}
      % \vspace{-6pt}
      \caption{\textbf{Data distributions.} We do vision-action instruction pre-training for \Ours on a dataset built upon Open X-Embodiment~\cite{open_x_embodiment_rt_x_2023}, including 8.5M image-2-D visual trace pairs.
      }
      \label{fig:supp:dataset}
    \end{figure*}
}


\def\emergentprop#1{
    \captionsetup[sub]{font=small}
    \begin{figure*}[#1]
      \centering
      \includegraphics[width=\linewidth]{Figure/emergent_properties.pdf}
      % \vspace{-6pt}
      \caption{\textbf{Emergent Properties:} \textbf{Top}: The task in this episode is ``take the steak off the grill". As we see in the third image, LLARVA fails to pick up the steak in the first attempt. However, it tries again and succeeds the second time, showing capability of attempting a task multiple times. \textbf{Bottom}: The single view which is used as the model input shows the top and back of a safe. The task is for the robot to move the money stack from the top of the safe to one of the shelves inside the safe. {\smodel} can still move the money to the correct shelf in the safe despite the camera view not showing the shelves.} 
      
      \label{fig:supp:emergent_prop}
    \end{figure*}
}



\def\figtrace#1{
    \captionsetup[sub]{font=small}
    \begin{figure*}[#1]
      \centering
      \includegraphics[width=\linewidth]{Figure/2dtrace.pdf}
      % \vspace{-6pt}
      \caption{We visualize the ground truth (yellow line), and \textbf{predicted 2-D visual trace (green dash line)} after we fine-tune our pre-trained model on specific downstream tasks. Our predicted 2-D visual trace gives reasonable route planning to achieve the goal, even sometimes diverge from the ground truth.}
      \label{fig:supp:2dtrace}
    \end{figure*}
}

\def\realsetup#1{
    \captionsetup[sub]{font=small}
    \begin{figure*}[#1]
      \centering
      \includegraphics[width=0.7\linewidth]{Figure/realsetup.png}
      % \vspace{-6pt}
      \caption{The real robot setup with Franka Emika Panda used for evaluating LLARVA.}
      \label{fig:realsetup}
    \end{figure*}
}

\def\suppdata#1{
    \captionsetup[sub]{font=small}
    \begin{figure*}[#1]
      \centering
      \includegraphics[width=\linewidth]{Figure/supp_data.pdf}
      % \vspace{-6pt}
      \caption{\textbf{A few samples from our constructed vision-action tuning dataset.} We visualize some samples of the instruction tuning dataset used in the pre-training stage of {\smodel}, with the corresponding robot type and control mode. }
      \label{supp:data}
    \end{figure*}
}

\def\Datatable#1{
\begin{table}[#1]
\tablestyle{10pt}{1.3}
\begin{center}
\setlength{\arrayrulewidth}{0.5mm}
\begin{tabular}{|l|l|}
\shline
\textbf{OXE Subset}                                                         & \multicolumn{1}{l|}{\textbf{Number of Image + 2-D visual trace pairs}} \\ \shline
kuka                                                                 & 1044466                                                     \\ \shline
austin\_sailor\_dataset\_converted\_externally\_to\_rlds             & 70758                                                       \\ \shline
fractal20220817\_data                                                & 753647                                                      \\ \shline
maniskill\_dataset\_converted\_externally\_to\_rlds                  & 909568                                                      \\ \shline
cmu\_play\_fusion                                                    & 47115                                                       \\ \shline
bc\_z                                                                & 1198963                                                     \\ \shline
berkeley\_rpt\_converted\_externally\_to\_rlds\_new                  & 1533451                                                     \\ \shline
bridge                                                               & 195745                                                      \\ \shline
language\_table                                                      & 885876                                                      \\ \shline
stanford\_kuka\_multimodal\_dataset\_converted\_externally\_to\_rlds & 30128                                                       \\ \shline
robo\_net                                                            & 496454                                                      \\ \shline
toto                                                                 & 65527                                                       \\ \shline
furniture\_bench\_dataset\_converted\_externally\_to\_rlds           & 786692                                                      \\ \shline
stanford\_hydra\_dataset\_converted\_externally\_to\_rlds            & 72160                                                       \\ \shline
ucsd\_pick\_and\_place\_dataset\_converted\_externally\_to\_rlds     & 13545                                                       \\ \shline
kaist\_nonprehensile\_converted\_externally\_to\_rlds                & 6512                                                        \\ \shline
stanford\_mask\_vit\_converted\_externally\_to\_rlds                 & 57012                                                       \\ \shline
utokyo\_pr2\_opening\_fridge\_converted\_externally\_to\_rlds        & 2276                                                        \\ \shline
berkeley\_fanuc\_manipulation                                        & 11854                                                       \\ \shline
utaustin\_mutex                                                      & 72461                                                       \\ \shline
taco\_play                                                           & 47780                                                       \\ \shline
berkeley\_autolab\_ur5                                               & 19621                                                       \\ \shline
austin\_sirius\_dataset\_converted\_externally\_to\_rlds             & 56101                                                       \\ \shline
columbia\_cairlab\_pusht\_real                                       & 5486                                                        \\ \shline
stanford\_robocook\_converted\_externally\_to\_rlds                  & 22894                                                       \\ \shline
roboturk                                                             & 37120                                                       \\ \shline
berkeley\_cable\_routing                                             & 7797                                                        \\ \shline
nyu\_franka\_play\_dataset\_converted\_externally\_to\_rlds          & 9118                                                        \\ \shline
jaco\_play                                                           & 15515                                                       \\ \shline
viola                                                                & 15146                                                       \\ \shline
tokyo\_u\_lsmo\_converted\_externally\_to\_rlds                      & 2398                                                        \\ \shline
austin\_buds\_dataset\_converted\_externally\_to\_rlds               & 6771                                                        \\ \shline
dlr\_sara\_pour\_converted\_externally\_to\_rlds                     & 2695                                                        \\ \shline
utokyo\_xarm\_pick\_and\_place\_converted\_externally\_to\_rlds      & 1381                                                        \\ \shline
utokyo\_pr2\_tabletop\_manipulation\_converted\_externally\_to\_rlds & 6545                                                        \\ \shline
dlr\_edan\_shared\_control\_converted\_externally\_to\_rlds          & 746                                                         \\ \shline
dlr\_sara\_grid\_clamp\_converted\_externally\_to\_rlds              & 1543                                                        \\ \shline
\end{tabular}
\vspace{0.2cm}
\caption{\textbf{More statistics about the vision-action instruction tuning dataset.}}
\label{supp:data_details}
\end{center}
\end{table}


}


\clearpage
\setcounter{page}{1}
\section*{Supplementary Material for ``LLARVA''}
% \maketitlesupplementary



% Here, we provide additional information about our experimental results, emergent properties, implementation details, and our constructed dataset. Specifically, \Secref{supp:expr} provides more experiment results, \Secref{supp:our:datasets} provides details about our constructed vision-action instruction dataset, \Secref{supp:impl} provides additional implementation details, and \Secref{supp:sec:emergent} shows emergent properties that can be observed from our model.

% Version that references the "Additional Experiments" section:
% Here, we provide additional information about our experimental results, emergent properties, implementation details, and our constructed dataset. Specifically, \Secref{supp:expr} provides more experiment results, \Secref{supp:our:datasets} provides details about our constructed vision-action instruction dataset, and \Secref{supp:impl} provides additional implementation details.


% Version that does NOT reference the "Additional Experiments" section:
Here, we provide additional information about our model's emergent properties, our constructed dataset, and implementation details. Specifically, \Secref{supp:sec:emergent} demonstrates interesting and unexpected model behaviors, \Secref{supp:our:datasets} provides details about our constructed vision-action instruction dataset, and \Secref{supp:impl} provides additional implementation details.



\section{Additional Experiment Results}
\label{supp:expr}



\def\tabsuppsimresults#1{
\begin{table}[#1]
\tablestyle{1.6pt}{1.2}
% \small
\begin{center}
\begin{tabular}{lcccccccccccc}

\multirow{2}{*}{Method} & \multicolumn{12}{c}{Task}\\
                        & \begin{tabular}[c]{@{}c@{}}open\\ drawer\end{tabular} & \begin{tabular}[c]{@{}c@{}}meat off\\ grill\end{tabular} & \begin{tabular}[c]{@{}c@{}}turn\\ tap\end{tabular} & \begin{tabular}[c]{@{}c@{}}put\\ money\end{tabular} & \begin{tabular}[c]{@{}c@{}}push\\ buttons\end{tabular} & \begin{tabular}[c]{@{}c@{}}sweep\\ dustpan\end{tabular} & \begin{tabular}[c]{@{}c@{}}slide\\ block\end{tabular} & \begin{tabular}[c]{@{}c@{}}close\\ jar\end{tabular} & \begin{tabular}[c]{@{}c@{}}screw\\ bulb\end{tabular} & \begin{tabular}[c]{@{}c@{}}place\\ wine\end{tabular} & \begin{tabular}[c]{@{}c@{}}reach and\\ drag\end{tabular} & \begin{tabular}[c]{@{}c@{}}stack\\ blocks\end{tabular} \\ \shline

                        \multicolumn{13}{c}{\color{gray}\textit{3-D methods}}   \\

\color{gray}C2FARM-BC               & \color{gray}20                                                    & \color{gray}20                                                       & \color{gray}68                                                 & \color{gray}12                                                  & \color{gray}72                                                     & \color{gray}0                                                       & \color{gray}16                                                    & \color{gray}24                                                  & \color{gray}8                                                    & \color{gray}18                                                   & \color{gray}24                                                       & \color{gray}0                                                      \\
\color{gray}PERACT                  & \color{gray}80                                                    & \color{gray}84                                                       & \color{gray}80                                                 & \color{gray}44                                                  & \color{gray}48                                                     & \color{gray}56                                                      & \color{gray}72                                                    & \color{gray}60                                                  & \color{gray}24                                                   & \color{gray}12                                                   & \color{gray}68                                                       & \color{gray}36                                                     \\ \hline

\multicolumn{13}{c}{\textit{2-D methods}}   \\

Image-BC (CNN)          & 4                                                     & 0                                                        & 8                                                  & 4                                                   & 0                                                      & 0                                                       & 4                                                     & 0                                                   & 8                                                    & 4                                                    & 0                                                        & 0                                                      \\ Image-BC (ViT)
                        & 0                                                     & 0                                                        & 16                                                 & 0                                                   & 0                                                      & 0                                                       & 0                                                     & 0                                                   & 16                                                   & 0                                                    & 0                                                        & 0                                                      \\ \hline

                        
\rowcolor{gray!10}LLARVA                  & \textbf{60}                                           & \textbf{80}                                              & \textbf{56}                                        & \textbf{44}                                         & \textbf{56}                                            & \textbf{84}                                             & \textbf{100}                                          & \textbf{28}                                         & \textbf{8}                                           & \textbf{12}                                          & \textbf{52}                                              & \textbf{0}                                            
\end{tabular}
\vspace{4pt}
\caption{\textbf{Success rate (\%) on RLBench Multi-Task setting.} We fine-tuned (with visual trace prediction) the pre-trained model on 12  tasks and evaluate with 25 episodes per task. Each evaluation episode is scored either 0 for failure or 100 for success. We \textcolor{gray}{gray out} methods with 3-D information.}
\vspace{-0.5cm}
\label{tab:supp-sim-main-results}
\end{center}
\end{table}
}



\subsection{Emergent Properties}
\label{supp:sec:emergent}
\emergentprop{htp}


\minisection{Multiple attempts after failure} The top row of~\cref{fig:supp:emergent_prop} shows an example of the model failing to pick up an object, and then retrying as soon as the end-effector comes back into view without the object in its grasp. Specifically, the third image represents the moment where the end-effector becomes visible again, and {\smodel} then attempts to complete the task again. This behavior emerges from the fact that the instruction prompt fed into {\smodel} at this moment is similar to the prompt at the start of the first attempt, with the main difference being the previous actions/positions included in the prompt. We highlight this as an interesting emergent property since the training data does not include any examples with such behavior. 

% For imitation learning, the model always has difficulties to do ``self-correction'', \ie if the prediction of a single step is not accurate and leads the motion deviated from the 

\minisection{Handling Obstructed Views}
In both pre-training and fine-tuning stages of {\smodel}, we use only a single camera view to provide visual inputs. Using only 2-D inputs creates a challenge since robotics tasks require very accurate action predictions in three dimensions. 

The model should be able to see the exact location of the target and also have a sense of depth, which other works typically achieve by using either multiple camera views or 3-D representations. We note that our model uses a single camera view due to input limitations of current open-source LMMs. These limitations can certainly be overcome and are left for future work. 

% In that perspective, the model should be able to see the exact location of the target and also have a great sense of depth which are achieved by adding more views in most of the work. 

Using a single camera view presents further challenges when objects in the scene occlude each other. However, we find that {\smodel} can often complete tasks even in these occluded situations. For example, as shown in the second row of~\cref{fig:supp:emergent_prop}, the task is \textit{``put the money away in the safe on the top shelf''}. The camera view only shows the top and back side of the safe, which is enough information to pick up the money from the top of the safe. However, the top shelf of the safe is not visible, and LLARVA can still predict the correct actions to place the stack of money there. This example shows {\smodel} can, in some cases, work despite visual obstructions, which we believe is in part attributable to the introduction of the visual traces. We hypothesize that understanding and predicting the visual trace provides the model with information about a successful end-effector trajectory in the presence of such occlusions.

% In our experiments, we are excited to find \Ours has potential to finish the job in a totally occluded case. For example, as shown in the second raw of~\cref{fig:supp:emergent_prop}, the task is \textit{``put the money away in the safe on the top shelf''}, our single view only covers the back side of the shelf. For picking the money, there is no issues for the model to know the exact location of the target, but after the money is picked, the end effector should go to the top shelf that are occluded or not covered in this scene. The experiment results show \Ours has potential ability to still work on that scenario, which we believe partly attributed to the introduction of the 2-D trace, which might provide additional information about where should the end effector go that compensate the lack of exact localization the occlusion brings.




% We present several additional experiments that further demonstrate the benefits of our {\smodel} approach. Shown in \cref{tab:supp-sim-main-results}, we provide results for a total of \giscard{correct this number for what we have by supp deadline} 18 simulator experiments (including the 12 experiments from \cref{tab:sim-main-results}).



% \subsection{Additional Experiments}
% \label{supp:more_ablt}

% % Here we provide additional results that {\smodel} achieves on RLBench tasks.
% \tabsuppsimresults{!htp}




%% ======================================================================================================

\section{Additional Dataset details}
\label{supp:our:datasets}

Here, we provide more information about our constructed dataset.
\Datatable{htp}

\figDatainfo{htp}
\suppdata{htp}

\minisection{Data Distribution} As mentioned in the paper, we construct the vision-action tuning dataset from a subset of Open X-Embodiment (OXE)~\cite{open_x_embodiment_rt_x_2023}. We excluded OXE subsets with poor image quality, smaller image resolution, ambiguous action spaces, or those with widely different robot morphologies such as Autonomous Mobile Robots (AMRs, which involve locomotion), resulting in ~8.5M image-text pairs, whose distribution is shown in~\cref{fig:supp:dataset} and \cref{supp:data_details}. Overall, we ensured that the resulting dataset contains subsets of~\cite{open_x_embodiment_rt_x_2023} that use end-effector control and joint control, in addition to including both absolute and delta control modes.

% The instruction tuning dataset consists of ~8.5M image-text pairs, and the distribution is made up of \giscard{verify the number of subsets} 13 subsets from OXE as detailed in ~\cref{fig:supp:dataset}. To maximize the variety of the dataset, we include all subsets except those with poor-quality images, small sizes, ambiguous action spaces, or completely different types of robots, such as Autonomous Mobile Robots (AMRs). We also include subsets that use end-effector control, joint control, and, similarly, both absolute and delta control modes. 


% \minisection{The Generation of 2-D Visual Traces} In order to generate 2-D visual traces, we trained an object detector to detect the end-effector given a 2-D image, and regarded the middle point of the bounding box as the keypoint of the end effector to generate the 2-D visual traces. We choose Faster R-CNN~\cite{girshick2015fast} implemented in detectron2~\cite{wu2019detectron2} as our object detector. For each subset, we randomly chose and annotated 200 images and used them to train the detector. We show some samples of our constructed data in~\cref{supp:data}. We visualize the 2-D visual traces as yellow lines on the visual observations. 

\minisection{The Generation of 2-D Visual Traces} The 2-D visual traces can be seen as a trace of the end-effector location in the image plane across time. To generate these traces, we trained an object detector to locate the end-effector from input 2-D images. We use the Detectron2~\cite{wu2019detectron2} implementation of Faster R-CNN~\cite{girshick2015fast} to obtain bounding boxes enclosing the end-effector, and then use the center point of the bounding boxes as the end-effector keypoint. The detector was trained using 200 manually annotated images from each OXE subset. Some examples of the resulting detector training set are shown in~\cref{supp:data}, where the 2-D visual traces are shown in yellow. Note that the traces are a sequence of 2-D coordinates, and \cref{supp:data} is a visualization of these sequences. During training the sequences are predicted in language token space and compared to ground truth.


\section{Additional Implementation Details}
\label{supp:impl}


\subsection{RLBench Experiments}
\Ours is evaluated on \giscard{replace with correct number of tasks} 12 tasks from RLBench. All RLBench tasks include two or more variations of a language instruction describing the goal.  For example, there might be three variations of the instruction for the same task: \textit{``open the top drawer'', ``grip the top handle and pull the top drawer open'' and ``slide the top drawer open''}. For simplicity, we use the first instruction variant for training. Below, we describe the RLBench tasks we use for simulator evaluation, along with any modifications we made to the tasks.  The intention behind the modifications is to increase the variations of the tasks, such as adding distractor objects with different colors. This exercises the model's language grounding abilities.

\minisection{Training Setup} We start with a {\smodel} model that has undergone vision-action instruction pre-training on OXE as described in \cref{subsec:training_step1}, and perform step 2 (\cref{subsec:training_step2}) instruction fine-tuning for four epochs on task-specific downstream data (e.g., picking, stacking, destacking) using eight A100 GPUs. Step 2 instruction tuning is done using 800 demonstrations for each RLBench task. The domain gap between step 1 and step 2 is large as we change from almost entirely real data to simulation while at the same time changing robots and tasks. We note that while other works train on a smaller amount of data, they use roughly the same order of magnitude of data as {\smodel}, and exploit the power of 3-D representations. For example, PerAct~\cite{shridhar2023perceiver} uses 100 examples per task but exploits voxel-based 3-D representations, which are rare and difficult to obtain. Our approach has the advantage of being able to leverage 2-D representations, which may require additional data but with roughly the same order of magnitude as methods that utilize 3-D.

\minisection{Open Drawer} The task is to open one of three drawers. The success metric is a full extension of the prismatic joint of the target drawer. We did not make any modifications to this task.

\minisection{Meat off Grill} The task is to take either a piece of chicken or steak off the grill and put it on the side. The success metric is the placement of the specified meat on the side, away from the grill. We did not make any modifications to this task.

\minisection{Turn Tap} The task is to turn either the left or right handle of the tap. Left and right are defined according to the orientation of the faucet. The success metric is the joint of the specified handle being at least $90^\circ$ away from the starting position. We did not make any modifications to this task.

\minisection{Put Money} The task is to pick up the stack of money and place it on the specified shelf of a safe. The safe has three shelves: top, middle, and bottom. The success metric is the placement of the stack of money on the specified shelf in the safe. We did not make any modifications to this task.

\minisection{Push Buttons} The task is to push the colored buttons in the specified sequence. There are always three buttons present in the scene, whose colors are sampled from 20 options, and the number of buttons to press is between one and three. The success metric is all specified buttons being pressed in the right order. We did not make any modifications to this task.

\minisection{Sweep Dustpan} The task is to sweep the dirt particles into the specified dustpan. There are two dustpans, one short and one tall, and both are always present in the scene. The success metric is all five dirt particles being inside the specified dustpan. We modified this task by adding a variation with a different-sized dustpan.


\minisection{Slide Block} In this task there is a block and four colored squares in the scene (green, blue, pink, and yellow). The task is to slide the block onto either the green or pink squares. The success metric used is some part of the block being on the specified target square. The original task only had one target square, and we modified it by adding three additional colored squares --- one target and two distractors.

\minisection{Close Jar}  The task is to screw in the lid on the jar with the specified color. There are always two colored jars in the scene, one target jar and one distractor jar. The success metric used is the lid being on top of the specified jar and the robot gripper not grasping any object. We modified this task so that the target jar color is drawn from a list of two possible colors (blue or teal). The color for the distractor jar was still chosen out of 20 options. 

\minisection{Screw Bulb} There are two bulb holders of different colors, and the task is to pick up a light bulb from the stand specified by color and screw it into the bulb stand. The color of the target holder is sampled from two colors, while the color of the distractor holder is sampled from the original 20 color options. The success metric used is the bulb from the specified holder being inside the bulb stand. We modified this task to use two colors for the target holder (yellow and purple) rather than 20 as in the original task specification. 

\minisection{Place Wine}  The task is to pick up the wine bottle and place it at the specified location in a wooden rack. The rack has three locations: left, middle, and right. The success metric is the placement of the bottle on the specified location in the rack. We did not make any modifications to this task.

\minisection{Reach and Drag} The environment has a cube, a stick, and four possible colored target squares. The task is to pick up the stick and use it to drag the cube to the target square of a specified color. The other three squares are considered distractors. The success metric used is some part of the block being inside the target's area. We modified this task to sample the target color from a list of three colors (maroon, magenta, teal). The colors for distractor squares are still sampled from 20 options.

\minisection{Stack Blocks } The scene starts with 8 blocks and a green platform. Four of the blocks are of a target color, and the other four have a distractor color. The task is to stack $N$ blocks of the target color on the green platform. The success metric is $N$ blocks being inside the area of the green platform. We did not make any modifications to this task.





\subsection{Real Robots Experiments} 

\minisection{Hardware Setup}
We use a Franka Emika Panda robot with a Franka gripper for real robot data collection and evaluations. A Logitech BRIO 4K camera positioned to the right of the Franka robot provides single-view RGB (without depth data) vision input to our model, as shown in Figure \ref{fig:realsetup}. Camera autofocus is disabled, and the data is captured at 640x480 resolution. The model inference is done on a 48GB NVIDIA A6000. 
\realsetup{h}



\minisection{Data Collection}
We use the data collection code and process from \hyperlink{https://github.com/Max-Fu/franka-scripted}{https://github.com/Max-Fu/franka-scripted} to collect data for picking, stacking, and destacking tasks. The script generates data for an arbitrary number of episodes. For each episode, the process generates x-y positions on the table plane using a uniform random distribution for each axis. The script directs the robot to place the cube at each location and then collects the camera and joint information as the robot is directed to pick, stack, or destack the cubes. Vision is not used during this process as the cube locations are all generated and therefore known. 

\minisection{Training and Execution}
For the Franka Emika Panda robot experiments, we start with our {\smodel} model that has undergone vision-action instruction pre-training on OXE as described in \cref{subsec:training_step1}, and perform step 2 (\cref{subsec:training_step2}) instruction fine-tuning for four epochs on 1920 episodes of task-specific downstream data (e.g., picking, stacking, destacking) using 8 A100 GPUs. This is similar to other baselines, such as RPT~\cite{radosavovic2023robot}, that uses an equal amount of in-domain episodes (1920) for pre-training, with an additional 120-240 episodes used for fine-tuning depending on the task. Additionally, \cite{radosavovic2023robot} uses three camera views for each episode, while {\smodel} uses only one. Nevertheless, it can be observed that {\smodel} demonstrates superior performance on all three tasks tested despite using comparable or even fewer episodes. 

% We note that our approach differs from other approaches in that in-domain data is not used during the pre-training stage, but only during the fine-tuning. Therefore, the total amount of in-domain data used to train our model is comparable to other approaches.


Each real robot evaluation consists of 16 repeated pick, stack, or destack operations at a random x-y location on the table plane for each repetition. We report the success rate of the 16 operations.

% \section{Qualitative Visualizations}
% \label{supp:qual}



\section{Licenses and Privacy}
\label{supp:datasets:Licenses}
The license, PII, and consent details of each dataset are in the respective papers. In addition, we wish to emphasize that the datasets we use do not contain any harmful or offensive content, as many other papers in the field also use them. Thus, we do not anticipate a specific negative impact, but, as with any machine learning method, we recommend exercising caution. 

